Transitions in magnetic behavior at the substellar boundary

We aim at advancing our understanding of magnetic activity and the underlying dynamo mechanism at the end of the main-sequence. To this end, we collected simultaneous X-ray and radio observations for a sample of M7-L0 dwarfs using XMM-Newton jointly with the JVLA and the ATCA. We also included data from the all-sky surveys of eROSITA on board the Russian Spektrum-Roentgen-Gamma mission (SRG) and rotation periods from TESS together with an archival compilation of X-ray and radio data for UCDs from the literature. We limit the sample to objects with rotation period <1d, focusing on the study of a transition in magnetic behavior suggested by a drastic change in the radio detection rate at vsini \approx 38 km/s. We compiled the most up-to-date radio/X-ray luminosity relation for 26 UCDs with rotation periods lower than 1d, finding that rapid rotators lie the furthest away from the G\"udel-Benz relation previously studied for earlier-type stars. Radio bursts are mainly experienced by very fast UCDs, while X-ray flares are seen along the whole range of rotation. We examined the L_{\rm x}/L_{\rm bol} vs P_{\rm rot} relation, finding no evident relation between the X-ray emission and rotation, reinforcing previous speculations on a bimodal dynamo across late-type dwarfs. One radio-detected object has a rotation period consistent with the range of auroral bursting sources; while it displays moderately circularly polarized emission. A radio flare from this object is interpreted as gyrosynchrotron emission, and it displays X-ray and optical flares. We also found a slowly rotating apparent auroral emitter, that is also one of the X-ray brightest radio-detected UCDs. We speculate that this UCD is experiencing a transition of its magnetic behavior since it produces signatures expected from higher mass M dwarfs along with emerging evidence of auroral emission.

==> Tables/Table_vlm_StellPar.tex <==
\begin{table*}
    \begin{center}
    \caption{Stellar properties of the literature sample (see Sect.~\ref{subsect:analysis_stepar}). Bolometric luminosities and radii (cols.3\&4) are calculated as for our UCDs sample \enmacomments{Beate, do you confirm?}. The values of $P_{\rm rot}$ shown in col.5 are computed with the analyisi of photometric data \citep{Crossfield2014} or upper limits calculated from the $v\cdot \sin{i}$ measurements. Results from {\it Gaia}-DR3 are shown from col.6 to 10. \textcolor{orange}{comment: I suggested to use the same format as for Table 2, and even to merge it. This will make it MUCH more easy for a reader to use the data in a future work. Believe me!} \enmacomments{If we want to this I have to readjust Table 1 as well, so moving the SpT too. Is it ok?}}
    \label{tab:lit_sample}
    \begin{tabular}{cccccccccc}
    \toprule[0.5mm]
      \multicolumn{1}{c}{Name} &
      \multicolumn{1}{c}{SpT} &
      \multicolumn{1}{c}{$\log L_{\rm bol}$} &
      \multicolumn{1}{c}{$R_{\star}$} &
      \multicolumn{1}{c}{$P_{\rm rot}$} &
      \multicolumn{1}{c}{GaiaID} &
      \multicolumn{1}{c}{Dist} &
      \multicolumn{1}{c}{$G$} &
      \multicolumn{1}{c}{$G_{\rm bp}$} &
      \multicolumn{1}{c}{$G{\rm rp}$} \\
      
      
       \multicolumn{1}{c}{} &
      \multicolumn{1}{c}{} &
      \multicolumn{1}{c}{[$L_{\odot}$]} &
      \multicolumn{1}{c}{[$R_{\odot}$]} &
      \multicolumn{1}{c}{[d]} &
      \multicolumn{1}{c}{} &
      \multicolumn{1}{c}{[pc]} &
      \multicolumn{1}{c}{[mag]} &
      \multicolumn{1}{c}{[mag]} &
      \multicolumn{1}{c}{[mag]} \\
    \midrule[0.5mm]
      2MJ0036 & L3.5 & -3.97 & 0.03 & 0.12 & 2794735086363871360 & 8.74$\pm$0.01 & 17.5 & 20.44 & 15.91 \\
      2MJ0523 & L2.5 & -3.78 & 0.03 & $<$0.09 & 2985035874544160384 & 12.73$\pm$0.02 & 18.03 & 21.27 & 16.48 \\
      2MJ0602 & L1.0 & -3.73 & 0.03 & $<$0.14 & 3457493517036545280 & 11.66$\pm$0.02 & 17.23 & 20.8 & 15.66 \\
      2MWJ1507 & L5.0 & -4.26 & 0.03 & $<$0.43 & 6306068659857135232 & 7.41$\pm$0.01 & 17.95 & 21.17 & 16.34 \\
      BRI0021-0214 & M9.5 & -3.44 & 0.12 & 0.17 & 2541756977144595712 & 12.45$\pm$0.03 & 16.58 & 20.02 & 15.03 \\
      DENIS J1048 & M9.0 & -3.53 & 0.1 & 0.25\enmacomments{$^{\rm Stef}$} & 5393446658454453632 & 4.05$\pm$0.01 & 14.01 & 17.62 & 12.46\\
      Gl 569 B & M9.1 & -3.17 & 0.15 & $<$0.40 & 1187851653287128576 & 9.94$\pm$0.01 & 9.12 & 10.31 & 8.03 \\
      Kelu 1 & L2.0 & -3.6 & 0.04 & 0.07 & 6187779556809793024 & 20.39$\pm$0.3 & 18.74 & 21.16 & 16.79 \\
      LHS2065 & M9.0 & -3.515 & 0.1 & $<$0.45 & 5761985432616501376 & 8.66$\pm$0.01 & 15.89 & 19.11 & 14.35 \\
      LHS3003\enmacomments{$^{\rm To~Be~Removed}$} & M7.0 & -3.19 & 0.12 & 2.01 & 6224387727748521344 & 7.05$\pm$0.01 & 14.06 & 17.34 & 12.57 \\
      LP 349-25 & M7.9 & -2.78 & 0.21 & 0.07 & 2799992744809482112 & 14.13$\pm$0.09 & 14.96 & 18.31 & 13.38 \\
      LP 412-31 & M7.9 & -3.26 & 0.12 & 0.61 & 56252256123908096 & 14.65$\pm$0.02 & 16.1 & 19.22 & 14.58 \\
      LP 944-20 & M9.5 & -3.84 & 0.07 & 0.16\enmacomments{$^{\rm Stef}$} & 4860376345833699840 & 6.43$\pm$0.01 & 15.44 & 18.94 & 13.89 \\
      LSR J1835 & M8.4 & -3.4 & 0.11 & 0.11 & 2091177593123254016 & 5.69$\pm$0.01 & 14.85 & 18.46 & 13.31 \\
      TVLM513 & M8.5 & -3.65 & 0.08 & 0.08 & 1262763648230973440 & 10.73$\pm$0.02 & 16.51 & 20.13 & 14.95 \\
      vB 10 & M8.0 & -3.39 & 0.1 & $<$0.80 & 4293315765165489536 & 5.92$\pm$0.01 & 14.3 & 17.75 & 12.77 \\
      vB 8 & M6.9 & -3.19 & 0.12 & $<$0.66 & 4339417394313320192 & 6.49$\pm$0.01 & 13.81 & 17.05 & 12.32 \\
    \bottomrule[0.5mm]
    \end{tabular}
    \end{center}


\end{table*}

